Clustering using skewed multivariate heavy tailed distributions with flexible tail behaviour

The family of location and scale mixtures of Gaussians has the ability to generate a number of flexible distributional forms. It nests as particular cases several important asymmetric distributions like the Generalised Hyperbolic distribution. The Generalised Hyperbolic distribution in turn nests many other well known distributions such as the Normal Inverse Gaussian (NIG) whose practical relevance has been widely documented in the literature. In a multivariate setting, we propose to extend the standard location and scale mixture concept into a so called multiple scaled framework which has the advantage of allowing different tail and skewness behaviours in each dimension of the variable space with arbitrary correlation between dimensions. Estimation of the parameters is provided via an EM algorithm with a particular focus on NIG distributions. Inference is then extended to cover the case of mixtures of such multiple scaled distributions for application to clustering. Assessments on simulated and real data confirm the gain in degrees of freedom and flexibility in modelling data of varying tail behaviour and directional shape.

==> preamble.tex <==

\usepackage{url}
\usepackage{graphicx}
\usepackage{amssymb,amsmath,enumerate}
\graphicspath{{pics/}{figs/}}
\usepackage{afterpage}
\usepackage{textcomp}
\RequirePackage{amsmath} \RequirePackage{xspace}

% DEFINITIONS PRELIMINAIRES
\def\argmax{\mathop{\mathrm{arg\,max}}} % Mieux que \def\argmax{\arg\max}
\def\argmin{\mathop{\mathrm{arg\,min}}} % car l'indice est reparti
\RequirePackage{amsmath} \RequirePackage{xspace}
\RequirePackage{bbm}


\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}
\def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}
\def\ellb{{\sbm{\ell}}\XS}

% ALPHABET GREC GRAS, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}
\def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}    \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}                 \def\Xib        {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}                 \def\Pib        {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}  \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib       {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib       {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}
\def\upsilonb       {{\sbmm{\upsilon}}\XS}
\def\PM{\kern0pt^{\textrm{{\scriptsize PM}}}\kern0pt}
\def\MMAP{\kern1pt^{\textrm{{\tiny MMAP}}}\kern-1pt}
\def\ML{^{\textrm{{\tiny ML}}}}
\def\dd{\,d}                            % doit etre en italique en anglais
\def\I{\,|\,}           % "sachant" bien espac\'e pour les formules


\newcommand{\w}{\omega}
\newcommand{\g}{\mathcal{G}}
\newcommand{\scalarprod}[2]{{{\bf \langle} {#1},{#2} {\bf \rangle}}}

\newcommand{\Hcondtheta}{H_{\theta\vert Y, T, S}} % loi conditionnelle
\newcommand{\HcondS}{H_{T \vert  S, Y, \theta}} % loi conditionnelle
\newcommand{\HcondT}{H_{S \vert T, Y, \theta}} % loi conditionnelle
\newcommand{\pjcomp}{p_{(Y,S,T)}} %  vraisemblance jointe complete.
\newcommand{\pjcondS}{p_{T \vert S, Y}} % loi conditionnelle
\newcommand{\pjcondT}{p_{S \vert T, Y}} % loi conditionnelle
\newcommand{\pjattach}{p_{Y \vert T, S}} % loi attache donnees
\newcommand{\pjpost}{p_{T, S \vert Y}} % loi a posteriori
\newcommand{\prior}{p_{Z}} % Loi a priori.
\newcommand{\pcomp}{p_{(Y,Z)}} %  vraisemblance complete.
\newcommand{\ppost}{p_{Z \vert Y}} % loi a posteriori
\newcommand{\pattach}{p_{Y \vert Z}} % loi a posteriori
\newcommand{\pinc}{p_{Y}} %  vraisemblance incomplete.
\newcommand{\KL}{\mathrm{KL}} % Distance de Kullback-Leibler
\newcommand{\Nv}{\mathcal{N}} %  voisinage
\newcommand{\DZe}{\mathcal{D}} % Ensemble des probabilites sur Z
\newcommand{\Ind}{\mathcal{I}} % Ensemble des probabilites independantes sur Z
\newcommand{\IndR}{\mathcal{I}_r} % Ensemble des probabilites independantes sur Z + restrictions
%% espaces de probabilites
\def\Prob{\mathbb{P}} % probabilite sur l'espace de la chaine
\def\Exp{\mathbb{E}} % esperance sur l'espace de la chaine
\def\BarExp{\bar{\mathbb{E}}} % esperance sur l'espace  de l'algo
\def\pbar{\bar{\mathbb{P}}} % probabilite sur l'espace de l'algo
%% variables al�atoires et realisations
\newcommand{\tv}{\ensuremath{\mathbf{t}}} % Vecteur des var cachees.(obs)
\newcommand{\sv}{\ensuremath{\mathbf{s}}} % Vecteur des var cachees.(obs)
\newcommand{\Tv}{\ensuremath{\mathbf{T}}} % Vecteur des var cachees.(obs)
\newcommand{\Sv}{\ensuremath{\mathbf{S}}} % Vecteur des var cachees.(obs)
\newcommand{\Wv}{\ensuremath{\mathbf{W}}} % Vecteur des var observees.(obs)
\newcommand{\wv}{\ensuremath{\mathbf{w}}} % Vecteur des var observees.(obs)
\newcommand{\Xv}{\ensuremath{\mathbf{X}}} % Vecteur des var observees.(obs)
\newcommand{\xv}{\ensuremath{\mathbf{x}}} % Vecteur des var observees.(obs)
\newcommand{\Yv}{\ensuremath{\mathbf{Y}}} % Vecteur des var observees.(obs)
\newcommand{\Zv}{\ensuremath{\mathbf{Z}}} % Vecteur des var cachees.(obs)
\newcommand{\yv}{\ensuremath{\mathbf{y}}} % Vecteur des var observees.(obs)
\newcommand{\zv}{\ensuremath{\mathbf{z}}} % Vecteur des var cachees.(obs)
\newcommand{\Ze}{\mathcal{Z}} % Espace d'etat du processus cach\'e.
\newcommand{\B}{{\cal B}}
\newcommand{\taubig}{{\cal T}}
\newcommand{\Be}{\underline{{\cal B}}}
\newcommand{\Phie}{\underline{\Phi}}
\newcommand{\zero}{\ensuremath{\mathbf{0}}}
\def\t{\theta} %parametre
%% Symboles generaux
\def\NNset{\mathbb{N}} % entiers  naturels
\def\Nset{\mathbb{Z}_+} % entiers  naturels
\def\Rset{\mathbb{R}} % reels
%\def\zero{{\mbox{\rm 0\hspace{-0.35em}0}}}  %
\def\un{{\mbox{\rm 1\hspace{-0.25em}I}}}  % indicatrice
\def\ie{\textit{i.e.} } % id est
\def\wp1{\mathrm{w.p.} 1}  % with respect to
%\newcommand{\etal}{{\em et al.}} % et al.
%%  GESTION DES DIALOGUES entre AUTEURS
\newenvironment{commentG}
 {\begin{quote}\color{green}\begin{sffamily}}
 {\end{sffamily}\color{black}\end{quote}}
%

